Measurement of the production cross-section of positive pions in the collision of 8.9 GeV/c protons on beryllium

The double-differential production cross-section of positive pions, $d^2\sigma^{\pi^{+}}/dpd\Omega$, measured in the HARP experiment is presented. The incident particles are 8.9 GeV/c protons directed onto a beryllium target with a nominal thickness of 5% of a nuclear interaction length. The measured cross-section has a direct impact on the prediction of neutrino fluxes for the MiniBooNE and SciBooNE experiments at Fermilab. After cuts, 13 million protons on target produced about 96,000 reconstructed secondary tracks which were used in this analysis. Cross-section results are presented in the kinematic range 0.75 GeV/c < $p_{\pi}$ < 6.5 GeV/c and 30 mrad < $\theta_{\pi}$ < 210 mrad in the laboratory frame.

==> abstract.tex <==


\begin{abstract}

The double-differential production 
cross-section of positive pions,\ \ddpiplus, measured in the HARP experiment is presented.  
The incident particles are 8.9 \GeVc\ protons directed onto a beryllium target with a 
thickness of  5\% of a nuclear interaction length.  
The measured cross-section has a direct impact on the prediction of neutrino fluxes for the 
MiniBooNE and SciBooNE experiments at Fermilab.  After cuts, 13 million protons on target
produced about 96,000 reconstructed secondary tracks which were used in this analysis.  
Cross-section results are presented in the kinematic range
0.75~\GeVc  $\leq p_{\pi} \leq$ 6.5~\GeVc 
and 30~mrad $\leq \theta_{\pi} \leq$ 210~mrad in the laboratory frame.  

\end{abstract} 

